Pre-shared Key Agreement for Secure Public Wi-Fi

This paper presents a novel pre-shared key (PSK) agreement scheme to establish a secure connection between a Wi-Fi client and access point (AP) without prior knowledge of a password. The standard IEEE 802.11 security method, Robust Security Network Association, widely known as Wi-Fi Protected Access (WPA) and WPA2, derives a shared cryptographic key if and only if a user provides an identical password which an AP possesses, causing ofinconvenience of obtaining and entering the password. In this paper, a proposed scheme, Secure Open AP (SOAP), adopts two public key algorithms, the elliptic curve Diffie-Hellman key exchange algorithm (ECDH) and digital signature algorithm (ECDSA) to establish a secure connection between a client and an AP without having prior knowledge of a password. Implementation and experiment results demonstrate the viability of the proposed scheme.

==> includes/acknowledgement.tex <==
\section*{Acknowledgements}

==> includes/table-auth-enc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{
  Classification of security protocols by authentication and cryptography
}
\label{tab:auth-enc}
\begin{tabular}{cc|cc}
\hline
                            &     & \multicolumn{2}{c}{Authentication} \\
                            &     & No                   & Yes         \\
\hline
\multirow{2}{*}{Cryptography} & No  & Open system                  & -         \\
                            & Yes & \textbf{Proposed scheme}      & WPA-PSK         \\
\hline
\end{tabular}
\end{table}


==> includes/table-wpa-term.tex <==
\begin{table}[h]
  \centering
  \caption{Terminologies used in WPA key exchange procedure and \nameshort{}}
  \label{tab:wpa-term}
  \begin{tabular}{rl}
    \hline
    % PSK & Pre-shared key \\
    % EAPOL & EAP over LAN \\
    Nonce & Random number used once on each side \\
    MIC & Message integrity code (checksum) \\
    % PTK & Pairwise transient key for unicast frame\\
    GTK & Group temporal key for broad/multicast frame\\
    PRF($\cdot$) & Pseudorandom function using SHA-1 \\%\cite{rfc2104}\\
    signature($\cdot$) & ECDSA signing function using SHA-256\\
    \hline
  \end{tabular}
\end{table}


==> includes/usecase.tex <==
\color{red}
\section{Use cases}
\label{sec:usecase}

We can find some practical use cases of \nameshort{}
for different purposes and scales.

\subsection{One stop installation of AP}

In a small area such as home, for people who are not familiar with electronic
devices, it is oftentimes difficult to install and setup an AP with security
feature, WPA/WPA2-PSK enabled.
Or even they may forget a password previously set.
In such a case, the proposed scheme can provide a convenient way to connect to
an APa but still can provide a secure communication.

\subsection{Store promotion with \namelong{}}

Recently, lots of stores such as Starbucks and Walmart
provide a freely accessible AP as a part of their promotions.
According to their policies, different authentication and encryption schemes are used.
OSA  is convenient to access but insecure, while WPA/WPA2-PSK is secure
but need to ask for a password even if there is no cost for it.
The propose scheme can be effective to both cases.
The proposed scheme adds encryption functionality to the former
and enables users to connect to an AP in the latter case.

\subsection{Global secure wireless network}

Major companies are making efforts to provide free APs in developing or
underdeveloped areas for wide spread and growth of information and
communications technology.
Google Station is one the most well-known project \cite{google-station}.
Currently, it deploys free APs to each railway station across India.
To use such APs, a user needs to follow SMS authentication on a web page.
However, it is for access control and irrelevant to WPA/WPA2 authentication procedure.
A connection between the AP and the user is still insecure.
In this case, the proposed scheme can precede SMS authentication.
Finally, the user can get a secure channel and an AP provider, Google, in this case,
still can control an individual's access.
\color{black}

